Booster: a Benchmark for Depth from Images of Specular and Transparent Surfaces

Estimating depth from images nowadays yields outstanding results, both in terms of in-domain accuracy and generalization. However, we identify two main challenges that remain open in this field: dealing with non-Lambertian materials and effectively processing high-resolution images. Purposely, we propose a novel dataset that includes accurate and dense ground-truth labels at high resolution, featuring scenes containing several specular and transparent surfaces. Our acquisition pipeline leverages a novel deep space-time stereo framework, enabling easy and accurate labeling with sub-pixel precision. The dataset is composed of 606 samples collected in 85 different scenes, each sample includes both a high-resolution pair (12 Mpx) as well as an unbalanced stereo pair (Left: 12 Mpx, Right: 1.1 Mpx), typical of modern mobile devices that mount sensors with different resolutions. Additionally, we provide manually annotated material segmentation masks and 15K unlabeled samples. The dataset is composed of a train set and two test sets, the latter devoted to the evaluation of stereo and monocular depth estimation networks. Our experiments highlight the open challenges and future research directions in this field.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> table/mono_vs_stereo.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}
 &
\multicolumn{2}{c}{All-Pixels} \\
\begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrr|r}
 \toprule
 $\delta$ $>$ 1.25 & $\delta$ $>$ 1.15 & $\delta$ $>$ 1.05& Abs. Rel \\
 $\uparrow$ (\%) & $\uparrow$ (\%) & $\uparrow$ (\%) & $\downarrow$ \\
 \midrule
 \\
 \midrule
 \\
 \\
 \\
 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrr|r}
 \toprule
 $\delta$ $>$ 1.25 & $\delta$ $>$ 1.15 & $\delta$ $>$ 1.05& Abs. Rel \\
 $\uparrow$ (\%) & $\uparrow$ (\%) & $\uparrow$ (\%) & $\downarrow$ \\
 \midrule
 0,986 & 0,964 & 0,825 & 0,057 \\
 \midrule
 0,063 & 0,997 & 0,988 & 0,915 \\
 0,983 & 0,946 & 0,756 & 0,054 \\
 1,000 & 0,924 & 0,715 & 0,053 \\
 0,951 & 0,899 & 0,639 & 0,084 \\
 \bottomrule
 \end{tabular} \\
 & CREStereo \cite{li2022practical} & DPT \cite{Ranftl_2021_ICCV} \\
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Stereo Test split -- material segmentation.} We run DPT \cite{midas} and CREStereo \cite{li2022practical}, using weights made available by their authors and process images at the resolution suggested by each network. We evaluate on full resolution ground-truth maps.}
 \label{tab:mono_vs_stereo}
\end{table}


==> table/segmentation_mono_dpt.tex <==
\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{ccc}

 % FULL RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Pre ft.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrr | rrr}
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 $\delta$ $<$ 1.25 & $\delta$ $<$ 1.15 & $\delta$ $<$ 1.05 & MAE & Abs. Rel & RMSE \\
 $\uparrow$ (\%) & $\uparrow$ (\%) & $\uparrow$ (\%) & $\downarrow$ (m) & $\downarrow$ & $\downarrow$ (m) \\
 \midrule
 97.51 & 94.14 & 78.69 & 0.083 & 0.069 & 0.112 \\
 \midrule
 99.26 & 96.22 & 81.14 & 0.085 & 0.068 & 0.114 \\ %10.12 & 8.20 & 13.24  \\
 96.83 & 93.41 & 81.72 & 0.090 & 0.078 & 0.104 \\ %10.28 & 9.01 & 11.68 \\
 93.65 & 84.68 & 57.58 & 0.092 & 0.097 & 0.112 \\ %5.99 & 6.34 & 7.10 \\
 88.22 & 81.20 & 65.68 & 0.093 & 0.100 & 0.108 \\  %8.85 & 9.66 & 10.17 \\ 
 \bottomrule
 \end{tabular}
 \\
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Post ft.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrr | rrr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 $\delta$ $<$ 1.25 & $\delta$ $<$ 1.15 & $\delta$ $<$ 1.05 & MAE & Abs. Rel & RMSE \\
 $\uparrow$ (\%) & $\uparrow$ (\%) & $\uparrow$ (\%) & $\downarrow$ (m) & $\downarrow$ & $\downarrow$ (m) \\
 \midrule
 97.83 & 94.82 & 79.04 & 0.079 & 0.065 & 0.106 \\
 \midrule
 96.36 & 97.31 & 82.36 & 0.082 & 0.066 & 0.108  \\
 89.28 & 93.71 & 81.05 & 0.091 & 0.079 & 0.102  \\
 98.38 & 90.31 & 68.54 & 0.074 & 0.078 & 0.089  \\
 90.67 & 85.03 & 70.60 & 0.078 & 0.082 & 0.090  \\ 
 \bottomrule
 \end{tabular}
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Mono benchmark -- material segmentation.} We run DPT \cite{Ranftl_2021_ICCV} processing images at the resolution suggested by the authors. Top: results using official weights. Bottom: results after fine-tuning using the Booster training split. We evaluate on full-resolution ground-truth maps.}
 \label{tab:segmentation_mono}
\end{table}


==> table/tables_old/segmentation_balanced_crestereo.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 (\%) & (\%) & (\%) & (\%) & (px.) &  (px.) \\
    33.07 & 21.36 & 17.35 & 15.09 & 12.56 & 29.45 \\
    \midrule     
    25.55 & 10.62 & 5.81 & 3.45 & 2.12 & 5.06 \\            
    36.31 & 21.38 & 15.95 & 12.82 & 5.62 & 12.13 \\           
    62.77 & 45.31 & 34.68 & 28.81 & 20.89 & 26.87 \\           
    79.50 & 69.29 & 62.08 & 56.19 & 53.34 & 66.73 \\ 
 \bottomrule
 \end{tabular}
 
 \\
 \\

 % QUARTER RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Quarter res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
    15.13 & 10.70 & 8.91 & 7.57 & 3.15 & 7.40 \\
    \midrule            
    3.49 & 1.55 & 0.82 & 0.57 & 0.54 & 1.30 \\           
    12.93 & 6.92 & 4.19 & 3.41 & 1.42 & 3.12 \\           
    28.90 & 18.76 & 16.66 & 15.66 & 5.25 & 6.82 \\           
    56.25 & 40.42 & 33.55 & 28.26 & 13.34 & 16.73 \\
 \bottomrule
 \end{tabular} \\
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Balanced benchmark -- material segmentation.} We run CRESTereo \cite{li2022practical }, using official weights, and process quarter-resolution images. We evaluate on full-resolution ground truths, or by downsampling them to quarter resolution.}
 \label{tab:segmentation_crestereo}
\end{table}

==> table/tables_old/segmentation_finetuning_balanced.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 (\%) & (\%) & (\%) & (\%) & (px.) &  (px.) \\
 \midrule
 38.68 & 23.33 & 17.66 & 14.55 & 7.56 & 17.39 \\
 \midrule
 37.50 & 20.47 & 13.75 & 10.40 & 4.43 & 10.07 \\
 42.48 & 23.35 & 16.15 & 12.22 & 5.24 & 12.05 \\
 61.84 & 42.37 & 33.23 & 27.37 & 13.08 & 18.08 \\
 65.59 & 48.74 & 39.19 & 32.93 & 14.91 & 21.75 \\ 
 \bottomrule
 \end{tabular}
 
 \\
 \\

 % FULL RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Quarter res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
 14.46 & 9.47 & 7.32 & 5.76 & 1.87 & 4.23 \\
 \midrule
 10.29 & 4.61 & 2.76 & 2.00 & 1.08 & 2.33 \\
 12.09 & 6.35 & 4.62 & 3.58 & 1.28 & 2.82 \\
 27.22 & 16.83 & 13.06 & 10.65 & 3.25 & 4.42 \\
 32.91 & 21.08 & 15.36 & 10.46 & 3.70 & 5.32 \\ 
 \bottomrule
 \end{tabular} 
 % &
 % \begin{tabular}{rrrr | rr }
 % \multicolumn{6}{c}{All pixels} \\
 % \toprule
 % bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 % $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 % \midrule
 %    30.59 & 17.57 & 13.10 & 10.87 & 6.78 & 16.44 \\
 %    \midrule           
 %    26.13 & 12.82 & 8.38 & 6.04 & 3.31 & 7.52  \\            
 %    33.59 & 17.51 & 12.14 & 9.83 & 5.19 & 11.13 \\           
 %    56.51 & 35.71 & 25.87 & 21.03 & 10.01 & 13.58 \\          
 %    66.98 & 49.29 & 39.17 & 32.47 & 21.94 & 30.41 \\   
 % \bottomrule
 % \end{tabular}
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Balanced benchmark after fine tuning -- material segmentation.} We run RAFT-Stereo, \textbf{fine-tuned} on the Booster training split, processing quarter resolution images. We evaluate on full resolution ground-truth maps or downsampled to quarter resolution.}
 \label{tab:finetuning}
\end{table}

==> table/tables_old/segmentation_finetuning_balanced_crestereo.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}

 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
    30.59 & 17.57 & 13.10 & 10.87 & 6.78 & 16.44 \\
    \midrule           
    26.13 & 12.82 & 8.38 & 6.04 & 3.31 & 7.52  \\            
    33.59 & 17.51 & 12.14 & 9.83 & 5.19 & 11.13 \\           
    56.51 & 35.71 & 25.87 & 21.03 & 10.01 & 13.58 \\          
    66.98 & 49.29 & 39.17 & 32.47 & 21.94 & 30.41 \\   
 \bottomrule
 \end{tabular}
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Balanced benchmark after fine tuning -- material segmentation.} We run CREStereo \cite{li2022practical}, \textbf{fine-tuned} by Booster training split, processing images at the lower camera resolution. We evaluate on full resolution ground truths maps.}
 \label{tab:finetuning_cres}
\end{table}

 \\
 \\


 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Quarter res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
    10.75 & 7.21 & 5.79 & 4.57 & 1.67 & 3.96 \\
    \midrule            
    5.87 & 3.19 & 2.21 & 1.74 & 0.80 & 1.64 \\            
    9.65 & 6.86 & 5.62 & 4.70 & 1.26 & 2.53 \\            
    20.82 & 12.33 & 9.90 & 8.43 & 2.47 & 3.25 \\            
    32.39 & 20.94 & 15.77 & 12.01 & 5.45 & 7.47 \\ 
 \bottomrule
 \end{tabular}
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Balanced benchmark after fine tuning -- material segmentation.} We run CREStereo \cite{li2022practical}, \textbf{fine-tuned} by Booster training split, processing images at the lower camera resolution. We evaluate on quarter resolution ground truths maps.}
 \label{tab:finetuning_cres}
\end{table}

==> table/tables_old/segmentation_finetuning_mono.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
 \begin{tabular}{c}
    \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
 \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrr | rrr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 $\delta$ $>$ 1.25 & $\delta$ $>$ 1.15 & $\delta$ $>$ 1.05 & MAE & Abs. Rel & RMSE \\
 $\uparrow$ (\%) & $\uparrow$ (\%) & $\uparrow$ (\%) & $\downarrow$ (m) & $\downarrow$ & $\downarrow$ (m) \\
 \midrule
 97.35 & 93.12 & 76.36 & 0.091 & 0.074 & 0.125  \\
 \midrule
 96.36 & 92.30 & 77.17 & 0.102 & 0.083 & 0.136  \\
 89.28 & 84.88 & 70.66 & 0.108 & 0.097 & 0.123  \\
 98.38 & 92.73 & 59.02 & 0.065 & 0.067 & 0.082  \\
 90.67 & 80.83 & 64.27 & 0.093 & 0.099 & 0.108  \\ 
 \bottomrule
 \end{tabular}
 
 \end{tabular}
 }
  \caption{\textbf{Results on the Booster Mono benchmark after fine tuning -- material segmentation.} We run MiDaS \cite{midas}, \textbf{fine-tuned} on the Booster training split, processing network resolution images. We evaluate on full resolution ground-truths.}
\label{tab:finetuning_midas}
\end{table}

==> table/tables_old/segmentation_finetuning_unbalanced.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
%  \begin{tabular}{c}
%     \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
%  \end{tabular}

 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
 58.67 & 32.83 & 22.96 & 17.65 & 6.31 & 11.11 \\
 \midrule
 57.04 & 27.58 & 17.36 & 12.97 & 4.72 & 7.14 \\
 53.17 & 30.29 & 22.32 & 17.13 & 5.16 & 7.83 \\
 61.90 & 40.06 & 31.54 & 26.18 & 6.71 & 10.00 \\
 61.40 & 42.12 & 32.50 & 26.79 & 10.56 & 14.64 \\ 
 \bottomrule
 \end{tabular}
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Unbalanced benchmark after fine tuning -- material segmentation.} We run RAFT-Stereo, \textbf{fine-tuned} by Booster training split, processing images at the lower camera resolution. We evaluate on full resolution ground truths maps.}
 \label{tab:unb_finetuning}
\end{table}




==> table/tables_old/segmentation_finetuning_unbalanced_crestereo.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
%  \begin{tabular}{c}
%     \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
%  \end{tabular}

 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$ (px.) \\
 \midrule
 53.86 & 27.25 & 17.98 & 12.99 & 5.19 & 9.34 \\    
 \midrule
 53.74 & 26.59 & 15.55 & 9.09 & 3.58 & 5.16 \\            
 52.65 & 24.88 & 14.29 & 9.47 & 3.98 & 6.21 \\            
 60.63 & 28.46 & 17.00 & 12.60 & 4.29 & 5.94 \\            
 59.65 & 37.56 & 27.61 & 21.36 & 10.48 & 14.57 \\ 
 \bottomrule
 \end{tabular}
 
 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Unbalanced benchmark after fine tuning -- material segmentation.} We run CREStereo \cite{li2022practical}, \textbf{fine-tuned} by Booster training split, processing images at the lower camera resolution. We evaluate on full resolution ground truths maps.}
 \label{tab:unb_finetuning_cres}
\end{table}

==> table/tables_old/segmentation_unbalanced_crestereo.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ccc}


 % FULL RESOLUTION TABLES
%  \begin{tabular}{c}
%     \multirow{3}{*}{\rotatebox{90}{Full res.}} \\ 
%  \end{tabular}
 \begin{tabular}{l}
 \\
 \toprule
 \\
 Category \\
 \midrule
 All \\
 \midrule
 Class 0 \\
 Class 1 \\
 Class 2 \\
 Class 3 \\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr }
 \multicolumn{6}{c}{All pixels} \\
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px.) & $\downarrow$  (px.) \\
 \midrule
 56.00 & 34.81 & 24.26 & 18.65 & 8.27 & 15.89 \\
 \midrule           
 52.33 & 30.42 & 19.40 & 12.93 & 5.21 & 6.85 \\           
 63.86 & 37.25 & 22.74 & 16.43 & 5.36 & 8.01 \\           
 66.79 & 39.00 & 20.49 & 14.80 & 7.36 & 9.36 \\            
 86.39 & 68.30 & 56.57 & 47.72 & 28.43 & 35.12 \\
 \bottomrule
 \end{tabular}

 \end{tabular}
 }
 \caption{\textbf{Results on the Booster Unbalanced benchmark -- material segmentation.} We run CRESTereo \cite{li2022practical}, using official weights. We process process images at the lower camera resolution. We evaluate on full resolution ground truths.}
 \label{tab:unb_segmentation_cres}
\end{table}
